Path-based Explanation for Knowledge Graph Completion

Graph Neural Networks (GNNs) have achieved great success in Knowledge Graph Completion (KGC) by modelling how entities and relations interact in recent years. However, the explanation of the predicted facts has not caught the necessary attention. Proper explanations for the results of GNN-based KGC models increase model transparency and help researchers develop more reliable models. Existing practices for explaining KGC tasks rely on instance/subgraph-based approaches, while in some scenarios, paths can provide more user-friendly and interpretable explanations. Nonetheless, the methods for generating path-based explanations for KGs have not been well-explored. To address this gap, we propose Power-Link, the first path-based KGC explainer that explores GNN-based models. We design a novel simplified graph-powering technique, which enables the generation of path-based explanations with a fully parallelisable and memory-efficient training scheme. We further introduce three new metrics for quantitative evaluation of the explanations, together with a qualitative human evaluation. Extensive experiments demonstrate that Power-Link outperforms the SOTA baselines in interpretability, efficiency, and scalability.

==> math_shortcuts.tex <==
% shortcuts for math symbols
\newcommand{\pvec}{\bm{u}}
\newcommand{\avec}{\bm{a}}
\newcommand{\graph}{\gG}
\newcommand{\compg}{\gG_{c}}
\newcommand{\edgeset}{\gR}
\newcommand{\nodeset}{\gE}
\newcommand{\model}{\mathcal{\phi}}
\newcommand{\parameteriser}{f}
\newcommand{\targettriplet}{\langle \hat{h}, \hat{r}, \hat{t}\rangle}
\newcommand{\triplet}{\langle e_i,r_j,e_k\rangle}
\newcommand{\pathset}{\gP}
\newcommand{\loss}{\gL}
\newcommand{\mask}{\gM}
\newcommand{\adj}{\mA}
\newcommand{\mpath}{\gS}



